Towards Multimodal Open-Set Domain Generalization and Adaptation through Self-supervision

The task of open-set domain generalization (OSDG) involves recognizing novel classes within unseen domains, which becomes more challenging with multiple modalities as input. Existing works have only addressed unimodal OSDG within the meta-learning framework, without considering multimodal scenarios. In this work, we introduce a novel approach to address Multimodal Open-Set Domain Generalization (MM-OSDG) for the first time, utilizing self-supervision. To this end, we introduce two innovative multimodal self-supervised pretext tasks: Masked Cross-modal Translation and Multimodal Jigsaw Puzzles. These tasks facilitate the learning of multimodal representative features, thereby enhancing generalization and open-class detection capabilities. Additionally, we propose a novel entropy weighting mechanism to balance the loss across different modalities. Furthermore, we extend our approach to tackle also the Multimodal Open-Set Domain Adaptation (MM-OSDA) problem, especially in scenarios where unlabeled data from the target domain is available. Extensive experiments conducted under MM-OSDG, MM-OSDA, and Multimodal Closed-Set DG settings on the EPIC-Kitchens and HAC datasets demonstrate the efficacy and versatility of the proposed approach. Our source code is available at https://github.com/donghao51/MOOSA.

==> tables/abla.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t!]
\begin{minipage}[t]{0.5\columnwidth}
\centering
\begin{adjustbox}{width=0.8\linewidth}

\begin{tabular}{l@{~~~~~}cccc  c}
\hline

         MulJig & MaskedTrans  & EntWei & \multicolumn{1}{c|}{EntMin}  &  \multicolumn{1}{c}{\textit{Mean} \textbf{\underline{HOS}}} \\
\hline

   & & &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{50.62}  \\

   $\checkmark$& & &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{51.88}  \\


   & $\checkmark$& &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{51.60}  \\


  $\checkmark$  & $\checkmark$& &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{53.91}  \\



  $\checkmark$  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{} & \multicolumn{1}{c}{54.77}  \\

    $\checkmark$ & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} &  \multicolumn{1}{c}{\textbf{55.38}}  \\


\hline
\end{tabular} 

\end{adjustbox}

\caption{Ablations of each proposed module in our \textit{MOOSA}.}


\label{tab:module}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\columnwidth}
\centering

\begin{adjustbox}{width=0.8\linewidth}
\begin{tabular}{l@{~~~~~}| c c}
\hline

   \multicolumn{1}{c|}{{Self-supervised Tasks}} & \multicolumn{1}{c}{\textit{Mean} \textbf{\underline{HOS}}} \\
\hline
% MSP

 %\multicolumn{1}{c|}{SimMMDG w/o CT} &\multicolumn{1}{c}{50.62}  \\
 
 \multicolumn{1}{c|}{Multimodal Alignment~\cite{Munro_2020_CVPR}} & \multicolumn{1}{c}{51.17}  \\
 
  \multicolumn{1}{c|}{Cross-modal Translation~\cite{dong2023SimMMDG}} & \multicolumn{1}{c}{48.94}  \\

  \multicolumn{1}{c|}{Relative Norm Alignment~\cite{Planamente_2022_WACV}} & \multicolumn{1}{c}{50.55}  \\
  
  \multicolumn{1}{c|}{Cross-modal Distillation~\cite{gupta2016cross}} & {50.88}  \\
 
 \multicolumn{1}{c|}{Masked Cross-moda Translation} &  \multicolumn{1}{c}{51.60}  \\

 
 \multicolumn{1}{c|}{Multimodal Jigsaw Puzzles} &   \multicolumn{1}{c}{51.88}  \\



 \multicolumn{1}{c|}{MaskedTrans+MulJig} &   \multicolumn{1}{c}{\textbf{53.91}}  \\

\hline

\end{tabular} 
\end{adjustbox}

\caption{Abation on different self-supervised tasks.}
\vspace{-1cm}

\label{tab:sst}
\end{minipage}
\end{table}




==> tables/abla2.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t!]
\begin{minipage}[t]{0.5\columnwidth}
\centering
\begin{adjustbox}{width=0.8\linewidth}

\begin{tabular}{l@{~~~~~}cccc  c}
\hline

         MulJig & MaskedTrans  & EntWei & \multicolumn{1}{c|}{EntMin}  &  \multicolumn{1}{c}{\textit{Mean} \textbf{\underline{HOS}}} \\
\hline

   & & &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{50.62}  \\

   $\checkmark$& & &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{51.88}  \\


   & $\checkmark$& &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{51.60}  \\


  $\checkmark$  & $\checkmark$& &  \multicolumn{1}{c|}{} &  \multicolumn{1}{c}{53.91}  \\



  $\checkmark$  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{} & \multicolumn{1}{c}{54.77}  \\

    $\checkmark$ & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} &  \multicolumn{1}{c}{\textbf{55.38}}  \\


\hline
\end{tabular} 

\end{adjustbox}

\caption{Ablations of each proposed module in our \textit{MOOSA}.}


\label{tab:module}
\end{minipage}
\hfill
\begin{minipage}[t]{0.5\columnwidth}
\centering

\begin{adjustbox}{width=0.8\linewidth}
\begin{tabular}{l@{~~~~~}| c c}
\hline

   \multicolumn{1}{c|}{{Self-supervised Tasks}} & \multicolumn{1}{c}{\textit{Mean} \textbf{\underline{HOS}}} \\
\hline
% MSP

 %\multicolumn{1}{c|}{SimMMDG w/o CT} &\multicolumn{1}{c}{50.62}  \\
 
 \multicolumn{1}{c|}{Multimodal Alignment~\cite{Munro_2020_CVPR}} & \multicolumn{1}{c}{51.17}  \\
 
  \multicolumn{1}{c|}{Cross-modal Translation~\cite{dong2023SimMMDG}} & \multicolumn{1}{c}{48.94}  \\

  \multicolumn{1}{c|}{Relative Norm Alignment~\cite{Planamente_2022_WACV}} & \multicolumn{1}{c}{50.55}  \\
  
  \multicolumn{1}{c|}{Cross-modal Distillation~\cite{gupta2016cross}} & {50.88}  \\
 
 \multicolumn{1}{c|}{Masked Cross-moda Translation} &  \multicolumn{1}{c}{51.60}  \\

 
 \multicolumn{1}{c|}{Multimodal Jigsaw Puzzles} &   \multicolumn{1}{c}{51.88}  \\



 \multicolumn{1}{c|}{MaskedTrans+MulJig} &   \multicolumn{1}{c}{\textbf{53.91}}  \\

\hline

\end{tabular} 
\end{adjustbox}

\caption{Abation on different self-supervised tasks.}
\vspace{-1cm}

\label{tab:sst}
\end{minipage}
\end{table}




==> tables/abla_para.tex <==

\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Parameters} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline


 \multicolumn{1}{c|}{0.9 4 64 1.0 0.5 0.1} &  40.90&88.24  & \multicolumn{1}{c|}{55.89}    &  43.37 & 62.50 & \multicolumn{1}{c|}{51.21}    &  43.85& 81.69 & \multicolumn{1}{c|}{57.07}    &  &  & \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{0.9 4 64 1.0 3.0 0.1} & 42.39 & 73.53 & \multicolumn{1}{c|}{53.78}    &  44.67 & 57.14 & \multicolumn{1}{c|}{50.14}    & 49.94& 64.79 & \multicolumn{1}{c|}{56.41}    &  &  & \multicolumn{1}{c}{}  \\
 
 
 \multicolumn{1}{c|}{0.9 4 64 1.0 0.3 0.1} & 43.14 & 61.76 & \multicolumn{1}{c|}{50.80}    & 40.92  & 58.93 & \multicolumn{1}{c|}{48.30}   &48.95  & 64.79 & \multicolumn{1}{c|}{55.77}     &  &  & \multicolumn{1}{c}{}  \\

 
 \multicolumn{1}{c|}{0.7 4 64 1.0 0.5 0.1} & 38.65 & 76.47 & \multicolumn{1}{c|}{51.35}    &  46.54 & 60.71 & \multicolumn{1}{c|}{52.69}   & 47.39 & 71.83 & \multicolumn{1}{c|}{57.11}     &  &  & \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{0.7 4 64 3.0 0.5 0.1} & 37.41&  73.53& \multicolumn{1}{c|}{49.59}    &  40.35 & 67.86 & \multicolumn{1}{c|}{50.60}   &46.84  & 67.61 & \multicolumn{1}{c|}{55.34}     &  &  & \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{0.7 4 64 0.5 0.5 0.1} & 42.64& 64.71 & \multicolumn{1}{c|}{51.41}    &  45.53 & 55.36 & \multicolumn{1}{c|}{49.97}   & 42.41 & 81.69 & \multicolumn{1}{c|}{55.84}     &  &  & \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{0.7 4 64 1.0 0.5 0.001} &42.39 & 64.71 & \multicolumn{1}{c|}{51.23}    &  41.64 & 66.07 & \multicolumn{1}{c|}{51.09}   &41.42  & 71.83 & \multicolumn{1}{c|}{52.54}     &  &  & \multicolumn{1}{c}{}  \\
 
 
 \multicolumn{1}{c|}{0.7 4 64 1.0 0.5 1.0} & 39.15&  73.53& \multicolumn{1}{c|}{51.10}    &   42.51& 64.29 & \multicolumn{1}{c|}{51.18}   & 42.75 & 69.01 & \multicolumn{1}{c|}{52.79}     &  &  & \multicolumn{1}{c}{}  \\
 
\hline

\end{tabular} 
}
\caption{Abation on different combination of parameters for multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-comb-abla} 
\end{table}

==> tables/epic-abla.tex <==
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}cccc ccc ccc ccc ccc}
\hline

\multicolumn{4}{c|}{\textbf{} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
         Jigsaw & MaskedTrans  & EntWei & \multicolumn{1}{c|}{EntMin} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline
% video audio



   & & &  \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{52.77}  &  &  & \multicolumn{1}{c|}{48.72}  &  &  & \multicolumn{1}{c|}{50.37}  &  &  & \multicolumn{1}{c}{50.62}  \\

   $\checkmark$& & &  \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{50.68}  &  &  & \multicolumn{1}{c|}{51.59}  &  &  & \multicolumn{1}{c|}{53.37}  &  &  & \multicolumn{1}{c}{51.88}  \\



   & $\checkmark$& &  \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{52.94}  &  &  & \multicolumn{1}{c|}{49.67}  &  &  & \multicolumn{1}{c|}{52.19}  &  &  & \multicolumn{1}{c}{51.60}  \\



  $\checkmark$  & $\checkmark$& &  \multicolumn{1}{c|}{} &  &  & \multicolumn{1}{c|}{51.14}  &  &  & \multicolumn{1}{c|}{53.78}  &  &  & \multicolumn{1}{c|}{56.81}  &  &  & \multicolumn{1}{c}{53.91}  \\



  $\checkmark$  & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{} & 46.63 & 64.71 & \multicolumn{1}{c|}{54.20}  &47.26  & 64.29 & \multicolumn{1}{c|}{54.48}  &  44.85& 73.24 & \multicolumn{1}{c|}{55.63}  &  &  & \multicolumn{1}{c}{54.77}  \\

    $\checkmark$ & $\checkmark$& $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} & 46.13 &   70.59 & \multicolumn{1}{c|}{55.80}  & 45.25 & 71.43  & \multicolumn{1}{c|}{55.40}  & 48.73 & 66.20 & \multicolumn{1}{c|}{56.69}  &  &  & \multicolumn{1}{c}{\textbf{55.96}}  \\



\hline
\end{tabular} 
}
\caption{Ablations of each proposed module on
EPIC-Kitchens dataset.}
\label{tab:epic-abla} 
\end{table}

==> tables/epic-da.tex <==



\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c c c c c c c  c}
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{1}{c|}{D1 $\rightarrow$ D2 } & \multicolumn{1}{c|}{D1 $\rightarrow$ D3 } & \multicolumn{1}{c|}{D2 $\rightarrow$ D1 } &\multicolumn{1}{c|}{D2 $\rightarrow$ D3 } & \multicolumn{1}{c|}{D3 $\rightarrow$ D1 } & \multicolumn{1}{c|}{D3 $\rightarrow$ D2 }  &  \multicolumn{1}{c}{\textit{Mean} }
 \\

\hline


 \multicolumn{1}{c|}{DeepAll}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{{MM-SADA~\cite{Munro_2020_CVPR}} } &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c}{}  \\

 
 \multicolumn{1}{c|}{{RNA-Net~\cite{Planamente_2022_WACV}}}&  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c}{}  \\

      
 \multicolumn{1}{c|}{{Audio-adaptive~\cite{ZhangCVPR2022}} } &  \multicolumn{1}{c|}{58.40}  &   \multicolumn{1}{c|}{54.20}  &   \multicolumn{1}{c|}{57.90}  & \multicolumn{1}{c|}{64.30}  &   \multicolumn{1}{c|}{55.90}  &  \multicolumn{1}{c|}{64.30}  &   \multicolumn{1}{c}{59.17}  \\
 
 \multicolumn{1}{c|}{{SimMMDG~\cite{dong2023SimMMDG}} } &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}  &   \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c}{}  \\

 
 \multicolumn{1}{c|}{{SimMMDG w/ Masked Translation+Jigsaw+EntWei+EntMin}} &  \multicolumn{1}{c|}{59.47}  &   \multicolumn{1}{c|}{59.03}  &   \multicolumn{1}{c|}{53.33}  & \multicolumn{1}{c|}{64.48}  &   \multicolumn{1}{c|}{}  &  \multicolumn{1}{c|}{}  &   \multicolumn{1}{c}{}  \\




\hline

\end{tabular} 
}
\caption{Multimodal \textbf{DA} with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-da} 
\end{table}

==> tables/epic-hyper-abla.tex <==



\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Mask ratio} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$\beta$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{0.1} & 40.65 &73.53 & \multicolumn{1}{c|}{52.35}  & 47.98 & 66.07 & \multicolumn{1}{c|}{55.59}  & 43.74 &71.83 & \multicolumn{1}{c|}{54.37}  & 44.12 & 70.48 & \multicolumn{1}{c}{54.10}  \\


 \multicolumn{1}{c|}{0.3} &  43.14& 58.82& \multicolumn{1}{c|}{49.78}  &  45.82&62.50  & \multicolumn{1}{c|}{52.88}  &  42.64&74.65 & \multicolumn{1}{c|}{54.27}  & 43.87 & 65.32 & \multicolumn{1}{c}{52.31}  \\

 \multicolumn{1}{c|}{0.5} &  39.40&73.53 & \multicolumn{1}{c|}{51.31}  & 45.82&62.50  & \multicolumn{1}{c|}{52.88}  &39.76  & 81.69& \multicolumn{1}{c|}{53.48}  & 41.66 & 72.57 & \multicolumn{1}{c}{52.56}  \\

 \multicolumn{1}{c|}{0.7} & 42.64 &73.53 & \multicolumn{1}{c|}{53.98}  & 50.29 & 67.86 & \multicolumn{1}{c|}{57.77}  & 45.52 & 67.61& \multicolumn{1}{c|}{54.40}  &46.15  & 69.67 & \multicolumn{1}{c}{55.38}  \\

 \multicolumn{1}{c|}{0.9} &42.14  &64.71 & \multicolumn{1}{c|}{51.04}  & 47.84 & 60.71 & \multicolumn{1}{c|}{53.51}  &  45.29&83.10 & \multicolumn{1}{c|}{58.63}  & 45.09 & 69.51 & \multicolumn{1}{c}{54.39}  \\


\hline

\end{tabular} 
}
\caption{Abation on different mask ratios $\beta$ for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-mask-abla} 
\end{table}





\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Jigsaw number} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$Q$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{32}   & 39.40 & 73.53 & \multicolumn{1}{c|}{51.31} & 43.52 & 71.43& \multicolumn{1}{c|}{54.08} & 46.40 & 69.01& \multicolumn{1}{c|}{55.49}  & 43.11 & 71.32 & \multicolumn{1}{c}{53.63}  \\


 \multicolumn{1}{c|}{64} & 42.64 & 64.71& \multicolumn{1}{c|}{51.41}  & 43.80 & 64.29 & \multicolumn{1}{c|}{52.10}  & 48.51 & 70.42& \multicolumn{1}{c|}{57.44}  &  44.98 & 66.47 & \multicolumn{1}{c}{53.65}  \\

 \multicolumn{1}{c|}{128} & 43.14 &58.82 & \multicolumn{1}{c|}{49.78}  & 45.82 &  62.50& \multicolumn{1}{c|}{52.88}  &  42.64&74.65 & \multicolumn{1}{c|}{54.27}  & 43.87 & 65.32 & \multicolumn{1}{c}{52.31}  \\

 \multicolumn{1}{c|}{256} &  45.14& 58.82& \multicolumn{1}{c|}{51.08}  & 48.42 & 58.93 & \multicolumn{1}{c|}{53.16}  &44.41  & 70.42& \multicolumn{1}{c|}{54.47}  &  45.99& 62.72 & \multicolumn{1}{c}{52.90}  \\

 \multicolumn{1}{c|}{512} &  42.39& 67.65& \multicolumn{1}{c|}{52.12}  & 48.13 & 55.36 & \multicolumn{1}{c|}{51.49}  & 50.61 & 61.97& \multicolumn{1}{c|}{55.72}  & 47.04 & 61.66 & \multicolumn{1}{c}{53.11}  \\


\hline

\end{tabular} 
}
\caption{Abation on different Jigsaw numbers $Q$ for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-Jigsaw-abla} 
\end{table}



\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Temperature } } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$T$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{0.3} & 41.65 & 79.41& \multicolumn{1}{c|}{54.64}  & 43.08 & 71.43 & \multicolumn{1}{c|}{53.75}  & 44.08 & 78.87& \multicolumn{1}{c|}{56.55}  & 42.94 & 76.57 & \multicolumn{1}{c}{54.98}  \\


 \multicolumn{1}{c|}{0.5} & 47.13 & 58.82& \multicolumn{1}{c|}{52.33}  & 55.04 & 60.71 & \multicolumn{1}{c|}{57.74}  & 48.17 & 67.61& \multicolumn{1}{c|}{56.26}  & 50.11 & 62.38 & \multicolumn{1}{c}{55.44}  \\

 \multicolumn{1}{c|}{0.7} & 44.39 & 64.71& \multicolumn{1}{c|}{52.66}  & 49.71 & 62.50 & \multicolumn{1}{c|}{55.38}  & 42.08 & 71.83 & \multicolumn{1}{c|}{53.07}  & 45.39 & 66.35 & \multicolumn{1}{c}{53.70}  \\

 \multicolumn{1}{c|}{1.0} &  43.14 &58.82 & \multicolumn{1}{c|}{49.78}  & 45.82 &  62.50& \multicolumn{1}{c|}{52.88}  &  42.64&74.65 & \multicolumn{1}{c|}{54.27}  &  43.87& 65.32 & \multicolumn{1}{c}{52.31}  \\

 \multicolumn{1}{c|}{3.0} & 43.89 & 64.71& \multicolumn{1}{c|}{52.30}  &  46.69& 75.00 & \multicolumn{1}{c|}{57.55}  & 42.75 & 78.87& \multicolumn{1}{c|}{55.44}  & 44.44 & 72.86 & \multicolumn{1}{c}{55.10}  \\

 
\hline

\end{tabular} 
}
\caption{Abation on different temperature values $T$ in entropy weighting for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-temp-abla} 
\end{table}






==> tables/epic-loss-abla.tex <==



\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$\alpha_1$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{0.01} & 44.14 & 61.76& \multicolumn{1}{c|}{51.49}  &  45.10& 69.64 & \multicolumn{1}{c|}{54.75}  &45.18  & 78.87& \multicolumn{1}{c|}{57.45}  & 44.81 & 70.09 & \multicolumn{1}{c}{54.56}  \\


 \multicolumn{1}{c|}{0.1} & 42.64 &73.53 & \multicolumn{1}{c|}{53.98}  & 50.29 & 67.86 & \multicolumn{1}{c|}{57.77}  & 45.52 & 67.61& \multicolumn{1}{c|}{54.40}  &46.15  & 69.67 & \multicolumn{1}{c}{55.38}  \\

 \multicolumn{1}{c|}{0.5} & 41.15 & 61.76& \multicolumn{1}{c|}{49.39}  & 46.97 & 58.93 & \multicolumn{1}{c|}{52.28}  & 44.74 &80.28 & \multicolumn{1}{c|}{57.46}  &44.29  & 66.99 & \multicolumn{1}{c}{53.04}  \\

 \multicolumn{1}{c|}{1.0} &40.40  &67.65 & \multicolumn{1}{c|}{50.59}  & 40.35 & 66.07 & \multicolumn{1}{c|}{50.10}  & 48.51 &61.97 & \multicolumn{1}{c|}{54.42}  &  43.09& 65.23 & \multicolumn{1}{c}{51.70}  \\



\hline

\end{tabular} 
}
\caption{Abation on different $\alpha_1$ for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-alpha1-abla} 
\end{table}





\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$\alpha_2$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{0.1}   & 43.39&64.71 & \multicolumn{1}{c|}{51.95}  & 41.07 & 76.79 & \multicolumn{1}{c|}{53.51}  & 49.72 & 64.79& \multicolumn{1}{c|}{56.26}  & 44.73 & 68.76 & \multicolumn{1}{c}{53.91}  \\


 \multicolumn{1}{c|}{0.5} & 39.65& 76.47& \multicolumn{1}{c|}{52.22}  & 47.84 & 55.36 & \multicolumn{1}{c|}{51.32}  &  46.95& 71.73& \multicolumn{1}{c|}{56.79}  & 44.81 & 67.85 & \multicolumn{1}{c}{53.44}  \\

 \multicolumn{1}{c|}{1.0} & 42.64 &73.53 & \multicolumn{1}{c|}{53.98}  & 50.29 & 67.86 & \multicolumn{1}{c|}{57.77}  & 45.52 & 67.61& \multicolumn{1}{c|}{54.40}  &46.15  & 69.67 & \multicolumn{1}{c}{55.38}  \\
 
 \multicolumn{1}{c|}{3.0} &  45.39 & 73.53& \multicolumn{1}{c|}{56.13}  &  40.78& 80.36 & \multicolumn{1}{c|}{54.10}  & 49.94 & 64.79& \multicolumn{1}{c|}{56.41}  & 45.37 & 72.89 & \multicolumn{1}{c}{55.55}  \\


\hline

\end{tabular} 
}
\caption{Abation on different $\alpha_2$ for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-alpha2-abla} 
\end{table}



\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{$\alpha_3$}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline

 \multicolumn{1}{c|}{0.001} & 46.13 &70.59 & \multicolumn{1}{c|}{55.80}  &  47.12& 58.93 & \multicolumn{1}{c|}{52.37}  & 43.52 &66.20 & \multicolumn{1}{c|}{52.52}  & 45.59 &  65.24& \multicolumn{1}{c}{53.56}  \\


 \multicolumn{1}{c|}{0.01} &45.14  &64.71 & \multicolumn{1}{c|}{53.18}  & 43.52 & 71.43 & \multicolumn{1}{c|}{54.08}  & 50.17 & 67.61& \multicolumn{1}{c|}{57.59}  &  46.28& 67.92 & \multicolumn{1}{c}{54.95}  \\

 \multicolumn{1}{c|}{0.1} & 42.64 &73.53 & \multicolumn{1}{c|}{53.98}  & 50.29 & 67.86 & \multicolumn{1}{c|}{57.77}  & 45.52 & 67.61& \multicolumn{1}{c|}{54.40}  &46.15  & 69.67 & \multicolumn{1}{c}{55.38}  \\

 \multicolumn{1}{c|}{1.0} &  43.64 &58.82 & \multicolumn{1}{c|}{50.11}  & 42.80 & 67.86 & \multicolumn{1}{c|}{52.49}  & 45.63 & 69.01& \multicolumn{1}{c|}{54.93}  & 44.02 & 65.23 & \multicolumn{1}{c}{52.51}  \\


 
\hline

\end{tabular} 
}
\caption{Abation on different $\alpha_3$ in entropy weighting for Multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-alpha3-abla} 
\end{table}






==> tables/epic-open-sst-ablation-deepall.tex <==
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Self-supervised} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{Tasks}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline
% MSP

 \multicolumn{1}{c|}{DeepAll} & 38.90 & 50.00 & \multicolumn{1}{c|}{43.76}  & 47.69 & 44.64 & \multicolumn{1}{c|}{46.12}  & 52.16 & 42.25 & \multicolumn{1}{c|}{46.69}  &  &  & \multicolumn{1}{c}{}  \\
 
\multicolumn{1}{c|}{Multimodal Alignment~\cite{Munro_2020_CVPR}} & 35.41 &  50.00 & \multicolumn{1}{c|}{41.46}  & 47.12 & 50.00 & \multicolumn{1}{c|}{48.52}  &51.16  & 46.48 & \multicolumn{1}{c|}{48.71}  &  &  & \multicolumn{1}{c}{}  \\
 
 \multicolumn{1}{c|}{Cross-modal Translation~\cite{dong2023SimMMDG}} & 46.63 & 47.06 & \multicolumn{1}{c|}{46.85}  & 51.44 & 44.64 & \multicolumn{1}{c|}{47.80}  &  45.40&  66.20& \multicolumn{1}{c|}{53.86}  &  &  & \multicolumn{1}{c}{}  \\

  \multicolumn{1}{c|}{Cross-modal Distillation} &  &  & \multicolumn{1}{c|}{}  &  &  & \multicolumn{1}{c|}{}  &  &  & \multicolumn{1}{c|}{}  &  &  & \multicolumn{1}{c}{}  \\
 
  \multicolumn{1}{c|}{Masked  Translation} & 44.14 & 55.88 & \multicolumn{1}{c|}{49.32}  & 46.83 & 50.00 & \multicolumn{1}{c|}{48.36}  & 48.28 & 60.56 & \multicolumn{1}{c|}{53.73}  &  &  & \multicolumn{1}{c}{}  \\

 
 \multicolumn{1}{c|}{Multimodal Jigsaw} & 39.65 & 50.00 & \multicolumn{1}{c|}{44.23}  & 44.81 & 50.00 & \multicolumn{1}{c|}{47.26}  & 41.41 & 56.34 & \multicolumn{1}{c|}{47.74}  &  &  & \multicolumn{1}{c}{}  \\




\hline

\end{tabular} 
}
\caption{Abation on different self-supervised tasks for multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-open-abla} 
\end{table}

==> tables/epic-open-sst-ablation.tex <==
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}| c ccc ccc ccc ccc}
\hline

 \multicolumn{1}{c|}{{Self-supervised} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
   \multicolumn{1}{c|}{{Tasks}} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline
% MSP

 \multicolumn{1}{c|}{SimMMDG w/o CT} &  &  & \multicolumn{1}{c|}{52.77}  &  &  & \multicolumn{1}{c|}{48.72}  &  &  & \multicolumn{1}{c|}{50.37}  &  &  & \multicolumn{1}{c}{50.62}  \\
 
 \multicolumn{1}{c|}{Multimodal Alignment~\cite{Munro_2020_CVPR}} &  &  & \multicolumn{1}{c|}{51.93}  &  &  & \multicolumn{1}{c|}{46.96}  &  &  & \multicolumn{1}{c|}{54.61}  &  &  & \multicolumn{1}{c}{51.17}  \\
 
  \multicolumn{1}{c|}{Cross-modal Translation~\cite{dong2023SimMMDG}} &  &  & \multicolumn{1}{c|}{46.27}  &  &  & \multicolumn{1}{c|}{49.18}  &  &  & \multicolumn{1}{c|}{51.37}  &  &  & \multicolumn{1}{c}{48.94}  \\

  \multicolumn{1}{c|}{Relative Norm Alignment~\cite{Planamente_2022_WACV}} & 36.16 & 85.29 & \multicolumn{1}{c|}{50.79}  & 44.24 & 58.93 & \multicolumn{1}{c|}{50.54}  & 40.09 & 67.61 & \multicolumn{1}{c|}{50.33}  &  &  & \multicolumn{1}{c}{50.55}  \\
  
  \multicolumn{1}{c|}{Cross-modal Distillation} &  &  & \multicolumn{1}{c|}{49.16}  &  &  & \multicolumn{1}{c|}{51.28}  &  &  & \multicolumn{1}{c|}{52.19}  &  &  & \multicolumn{1}{c}{50.88}  \\
 
 \multicolumn{1}{c|}{Masked  Translation} &  &  & \multicolumn{1}{c|}{52.94}  &  &  & \multicolumn{1}{c|}{49.67}  &  &  & \multicolumn{1}{c|}{52.19}  &  &  & \multicolumn{1}{c}{51.60}  \\

 
 \multicolumn{1}{c|}{Multimodal Jigsaw} &  &  & \multicolumn{1}{c|}{50.68}  &  &  & \multicolumn{1}{c|}{{51.59}}  &  &  & \multicolumn{1}{c|}{53.37}  &  &  & \multicolumn{1}{c}{\textbf{51.88}}  \\



\hline

\end{tabular} 
}
\caption{Abation on different self-supervised tasks for multimodal \textbf{Open-set} DG with video and audio modalities on EPIC-Kitchens dataset.}
\label{tab:epic-open-abla} 
\end{table}

==> tables/epic-open-test.tex <==
\begin{table}[t!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l@{~~~~~}cc ccc ccc ccc ccc ccc}
\hline

 & &\multicolumn{3}{c|}{\textbf{Modality} } &\multicolumn{3}{c|}{D2, D3 $\rightarrow$ D1 } & \multicolumn{3}{c|}{D1, D3 $\rightarrow$ D2 } & \multicolumn{3}{c|}{D1, D2 $\rightarrow$ D3 }  &  \multicolumn{3}{c}{\textit{Mean} }
 \\
        &  & Video  & Audio & \multicolumn{1}{c|}{Flow} & OS* & UNK & \multicolumn{1}{c|}{\textbf{\underline{HOS}}} &  OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c|}{\textbf{\underline{HOS}}}  & OS* & UNK &  \multicolumn{1}{c}{\textbf{\underline{HOS}}} \\
\hline


% audio flow
{DeepAll} &  & &$\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} & 40.90 & 44.12 & \multicolumn{1}{c|}{42.45}  & 46.25 & 37.50 & \multicolumn{1}{c|}{41.42}  & 38.32 & 46.48 & \multicolumn{1}{c|}{42.01}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\

{MM-SADA~\cite{Munro_2020_CVPR}} &  & &$\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} & 38.90 & 47.06 & \multicolumn{1}{c|}{42.59}  & 45.97 & 42.86 & \multicolumn{1}{c|}{44.36}  & 45.52 & 40.85 & \multicolumn{1}{c|}{43.05}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\

{RNA-Net~\cite{Planamente_2022_WACV}} &  &&  $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} & 37.16 & 52.94 & \multicolumn{1}{c|}{43.67}  & 46.69 & 46.43 & \multicolumn{1}{c|}{46.56}  &47.51  & 40.85 & \multicolumn{1}{c|}{43.93}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\

{SimMMDG~\cite{dong2023SimMMDG}} &  & & $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} & 43.64& 52.94 & \multicolumn{1}{c|}{ 47.84}  &  46.54& 67.86 & \multicolumn{1}{c|}{55.21}  &36.88  & 60.56 & \multicolumn{1}{c|}{45.84}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\

{SimMMDG+Jigsaw} &  && $\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} & 37.41 & 64.71 & \multicolumn{1}{c|}{47.41}  &46.54  &73.21  & \multicolumn{1}{c|}{56.91}  &39.31  & 59.15 & \multicolumn{1}{c|}{47.24}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\


{SimMMDG+Jigsaw+EntWei+EntMin}&  & & $\checkmark$&  \multicolumn{1}{c|}{$\checkmark$} & 37.91 & 64.71 & \multicolumn{1}{c|}{47.81}  & 47.26 & 76.79 & \multicolumn{1}{c|}{58.51}  & 39.31 &  69.01& \multicolumn{1}{c|}{50.09}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\


{SimMMDG w/ Masked Translation} &  & &$\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} & 36.91 & 67.65  & \multicolumn{1}{c|}{47.76}  & 49.57 & 64.29 & \multicolumn{1}{c|}{55.98}  & 38.10 & 61.97 & \multicolumn{1}{c|}{47.19}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\


{SimMMDG w/ Masked Translation+Jigsaw} &  & &$\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} &37.16 & 64.71 & \multicolumn{1}{c|}{47.21}  & 51.15 & 60.71 & \multicolumn{1}{c|}{60.03}  & 42.19 & 64.79 & \multicolumn{1}{c|}{51.10}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\


{SimMMDG w/ Masked Translation+Jigsaw+EntWei+EntMin } &  & &$\checkmark$ &  \multicolumn{1}{c|}{$\checkmark$} & 42.64 & 55.88 & \multicolumn{1}{c|}{48.37}  &  46.69& 75.00 & \multicolumn{1}{c|}{57.55}  &  42.19& 57.75 & \multicolumn{1}{c|}{48.76}  &  &  & \multicolumn{1}{c}{\textbf{}}  \\





\hline

\end{tabular} 
}
\caption{Multimodal \textbf{Open-set} DG with different combinations of modalities on EPIC-Kitchens dataset.}
\label{tab:epic-open} 
\end{table}
